A Geometric Perspective on First-Passage Competition

We study the macroscopic geometry of first-passage competition on the integer lattice $Z^d$, with a particular interest in describing the behavior when one species initially occupies the exterior of a cone. First-passage competition is a stochastic process modeling two infections spreading outward from initially occupied disjoint subsets of $Z^d$. Each infecting species transmits its infection at random times from previously infected sites to neighboring uninfected sites. The infection times are governed by species-specific probability distributions, and every vertex of $Z^d$ remains permanently infected by whichever species infects it first. We introduce a new, simple construction of first-passage competition that works for an arbitrary pair of disjoint starting sets in $Z^d$, and we analogously define a deterministic first-passage competition process in the Euclidean space $R^d$, providing a formal definition for a model of crystal growth that has previously been studied computationally. We then prove large deviations estimates for the random $Z^d$-process, showing that on large scales it is well-approximated by the deterministic $R^d$-process, with high probability. Analyzing the geometry of the deterministic process allows us to identify critical phenomena in the random process when one of the two species initially occupies the entire exterior of a cone and the other species initially occupies a single interior site. Our results generalize those in a 2007 paper of Deijfen and H\"aggstr\"om, who considered the case where the cone is a half-space. Moreover, we use our results about competition in cones to strengthen a 2000 result of H\"aggstr\"om and Pemantle about competition from finite starting configurations.

==> analysis.tex <==
% TeXShop Macros:
% !TEX TS-program = pdflatexmk
% !TEX root = thesis.tex

%I'm not really sure what I want to call this, or what will go in here, if anything...
\chapter{Analysis and Probability Proofs}
\label{analysis_chap}

\begin{lem}
\label{sufficient_moment_cond_lem}
\Lspace{1/2} implies \minimalmoment{d} for all $d\ge 1$.
\end{lem}

\begin{proof}
I think I have a proof of this in an old notebook somewhere, using some results in Folland\ldots Yes, at the back of my notebook from 2008, I think.
\end{proof}

{%Wrapper
\newcommand{\sigfield}{\mathcal{F}}
\begin{lem}
\label{zero_cond_prob_lem}
Let $\probabilityspace$ be a probability space, and let $A\in \sigmafield$ be an event. Then the following are equivalent.
\begin{enumerate}
\item $\Pr(A)>0$.
\item $\cprob{A}{\sigfield} >0$ $\Pr$-a.s.\ for some $\sigma$-field $\sigfield\subseteq \sigmafield$.
\item $\cprob{A}{\sigfield} >0$ $\Pr$-a.s.\ for all $\sigma$-fields $\sigfield\subseteq \sigmafield$.
\end{enumerate}
\end{lem}

\begin{proof}
Easy\ldots
\end{proof}
}%End wrapper

\begin{lem}[Large deviations estimate for \iid\ averages]
\label{basic_large_dev_lem}
\newcommand{\thisrv}{X}
\newcommand{\thislaw}{\law (\thisrv)}
\newcommand{\expconst}{b}

\newcommand{\thisC}{\bigcref{basic_large_dev_lem}}
\newcommand{\thisCp}[2][0]{\thisC \parens[#1]{#2}}
\newcommand{\thisc}{\smallcref{basic_large_dev_lem}}
\newcommand{\thiscp}[2][0]{\thisc \parens[#1]{#2}}

Let $\thisrv,\thisrv_1,\thisrv_2,\dotsc$ be \iid\ random variables such that $\E e^{b \thisrv} <\infty$ for some $b>0$. Then $\E\thisrv \in [-\infty,+\infty)$, and for any $x> \E\thisrv$, there are positive constants $\thisCp{x}$ and $\thiscp{x}$ (which depend on $\thislaw$) such that for any positive integer $n$,
\[
\Pr \eventthat[1]{\textstyle \frac{1}{n}\sum_{j=1}^n \thisrv_j \ge x}
\le \thisCp{x} e^{-\thiscp{x} n}.
\]
\end{lem}

\begin{proof}
This follows from basic large deviations theory. See for example Corollary~27.4 on p.\ 541 of Kallenberg.
\end{proof}

%%Commented out 2012/1/26.
%%I do an easier proof of a special case in the segment measure lemma, and then state another special case of this result without proof in the "line segments in a spherical shell" lemma.
%
%\begin{lem}[The number of lattice points in a cylindrical segment]
%\label{cyl_points_lem}
%\newcommand{\normone}{\mu_1}
%\newcommand{\normtwo}{\mu_2}
%
%\newcommand{\thispoint}{\vect x}
%\newcommand{\thisline}{L}
%
%\newcommand{\thisdir}{\dirvec}
%\newcommand{\thisray}{\thispoint+\thisdir}
%
%\newcommand{\thisvertex}{\vect v}
%
%\newcommand{\thisconst}{\normcylconst{\normone}{\normtwo}}
%
%\newcommand{\radius}{r}
%
%%%FIRST VERSION (Sat Jan 21, 2012)
%%%Commented out 2012/1/24
%%For any norms $\normone$ and $\normtwo$, there exists some constant $\thisconst$ such that if $\thispoint$ is any point in $\Rd$ and $\thisline$ is any line through $\thispoint$, then for any $r\ge 0$ and $0\le a\le b$,
%%\[
%%\card[1]{\setbuilder[1]{\thisvertex\in\Zd}
%%{\distnew{\normone}{\thisvertex}{\thisline} \le \radius
%%\text{\rm\ and } a\le \distnew{\normtwo}{\thisvertex}{\thispoint} \le b}}
%%\le \thisconst (\radius\join 1)^{d-1} \brackets[2]{(b-a)\join 1}
%%\]
%%[[Oops, unless $a=0$, this gives a pair of cylindrical segments rather than just one. Maybe use a ray instead\ldots]]
%
%%SECOND VERSION (Mon Jan 23, 2012)
%For any norms $\normone$ and $\normtwo$, there exists some constant $\thisconst$ such that if $\thispoint$ is any point in $\Rd$ and $\thisdir$ is any direction in $\dirset{\Rd}$, then for any $r\ge 0$ and $0\le a\le b$,
%%%==One line version:
%%\[
%%\card[1]{\setbuilder[1]{\thisvertex\in\Zd}
%%{\distnew{\normone}{\thisvertex}{\thisray} \le \radius
%%\text{\rm\ and } a\le \distnew{\normtwo}{\thisvertex}{\thispoint} \le b}}
%%\le \thisconst (\radius\join 1)^{d-1} \brackets[2]{(b-a)\join 1}
%%\]
%%==Two line version:
%\[
%\card[1]{\setbuilderbar[1]{\thisvertex\in\Zd}
%{\mathstack{\distnew{\normone}{\thisvertex}{\thisray} \le \radius \text{\rm\ and }}
%	{a\le \distnew{\normtwo}{\thisvertex}{\thispoint} \le b}}}
%\le \thisconst (\radius\join 1)^{d-1} \brackets[2]{(r\join 1)+(b-a)}
%\]
%
%\end{lem}
%
%\begin{proof}
%\newcommand{\normone}{\mu_1}
%\newcommand{\normtwo}{\mu_2}
%
%\newcommand{\thispoint}{\vect x}
%%\newcommand{\thisline}{L}
%
%\newcommand{\thisdir}{\dirvec}
%\newcommand{\thisray}{\thispoint+\thisdir}
%
%\newcommand{\thisvertex}{\vect v}
%
%\newcommand{\thisconst}{\normcylconst{\normone}{\normtwo}}
%
%\newcommand{\radius}{r}
%
%%==Additional commands:
%
%\newcommand{\vset}{V}
%\newcommand{\thiscyl}{C}
%
%\newcommand{\thisy}{\vect y}
%
%\newcommand{\dilsymb}{\Delta}
%\newcommand{\invdilsymb}{\delta}
%
%\newcommand{\thisdil}[2]{\dilsymb_{#1}^{#2}}
%\newcommand{\thisinvdil}[2]{\invdilsymb_{#1}^{#2}}
%
%\newcommand{\dilone}{\delta_1}
%\newcommand{\diltwo}{\delta_2}
%
%Let $\vset$ be the set of lattice points in the statement. Then $\card{\vset} = \lebmeasof{d}{\cubify{\vset}}$ by Lemma~\ref{lattice_cube_properties_lem}. Our strategy will be to find a Euclidean cylinder $\thiscyl$ containing $\cubify{\vset}$, and then compute the volume of $\thiscyl$. Since the Euclidean metric is isotropic and Lebesgue measure is invariant under isometries, this strategy will produce a bound that does not depend on the location $\thispoint$ or the direction $\thisdir$.
%
%Recall that $\cubify{\vset} = \vset+\frac{1}{2}\unitball{\linfty{d}}$, so if $\thisy\in \cubify{\vset}$, then there is some $\thisvertex\in\vset$ such that $\distnew{\linfty{d}}{\thisy}{\thisvertex}\le 1/2$. Thus, if we set $\thisdil{\infty}{\normone} \definedas \dilnorm{\linfty{d}}{\normone}$ and $\thisdil{\infty}{\normtwo} \definedas \dilnorm{\linfty{d}}{\normtwo}$, then
%%\begin{align*}
%%\cubify{\vset} \subseteq
%%\setbuilder[1]{\thisy\in \Rd}
%%{\distnew{\normone}{\thisy}{\thisray} \le \radius + \tfrac{1}{2}\thisdil{\infty}{\normone}
%%\text{\rm\ and } 
%%a - \tfrac{1}{2}\thisdil{\infty}{\normtwo} \le \distnew{\normtwo}{\thisy}{\thispoint}
%%	\le b + \tfrac{1}{2}\thisdil{\infty}{\normtwo}}.
%%\end{align*}
%\begin{align*}
%\cubify{\vset} \subseteq
%\setbuilderbar[1]{\thisy\in \Rd}{\mathstack
%	{\distnew{\normone}{\thisy}{\thisray} \le \radius + \tfrac{1}{2}\thisdil{\infty}{\normone}
%	\text{\rm\ and } }
%	{a - \tfrac{1}{2}\thisdil{\infty}{\normtwo} \le \distnew{\normtwo}{\thisy}{\thispoint}
%	\le b + \tfrac{1}{2}\thisdil{\infty}{\normtwo}}}.
%\end{align*}
%Now let $\thisdil{\normone}{2} \definedas \dilnorm{\normone}{\ltwo{d}}$, $\thisdil{\normtwo}{2} \definedas \dilnorm{\normtwo}{\ltwo{d}}$, and $\thisinvdil{\normtwo}{2} \definedas \dilnorm{\ltwo{d}}{\normtwo}^{-1} = \inf_{\vect z\ne \vect 0} {\norm{\vect z}_{\ltwo{d}}}/{\mu_2(\vect z)}$. Then using the fact that $\thisinvdil{\normtwo}{2} \le \thisdil{\normtwo}{2}$ in the second line, the above equation implies that
%\begin{align*}
%\cubify{\vset} &\subseteq
%\setbuilderbar[1]{\thisy\in \Rd}{\mathstack
%	{\distnew{\ltwo{d}}{\thisy}{\thisray} \le
%		\thisdil{\normone}{2} \parens{ \radius + \tfrac{1}{2}\thisdil{\infty}{\normone}}
%		\text{\rm\ and } }
%	{\thisinvdil{\normtwo}{2} \parens{a - \tfrac{1}{2}\thisdil{\infty}{\normtwo}}
%		\le \distnew{\ltwo{d}}{\thisy}{\thispoint}
%		\le \thisdil{\normtwo}{2} \parens{b + \tfrac{1}{2}\thisdil{\infty}{\normtwo}}}}\\
%&\subseteq \setbuilderbar[1]{\thisy\in \Rd}{\mathstack
%	{\distnew{\ltwo{d}}{\thisy}{\thisray} \le
%		\thisdil{\normone}{2} \parens{ \radius + \tfrac{1}{2}\thisdil{\infty}{\normone}}
%		\text{\rm\ and } }
%	{ a - \tfrac{1}{2}\thisdil{\infty}{\normtwo}
%		\le \frac{1}{\thisinvdil{\normtwo}{2}} \distnew{\ltwo{d}}{\thisy}{\thispoint}
%		\le \thisdil{\normtwo}{2} \parens{b + \tfrac{1}{2}\thisdil{\infty}{\normtwo}}}}.
%\end{align*}
%
%
%\[
%\vset \subseteq
%\setbuilder[1]{\thisvertex\in\Zd}
%{\distnew{\ltwo{d}}{\thisvertex}{\thisray} \le \dilone \radius
%\text{\rm\ and } a\le \distnew{\ltwo{d}}{\thisvertex}{\thispoint} \le b}
%\]
%
%\end{proof}

\begin{lem}[The number of lattice points in a spherical shell]
\label{norm_shell_lem}
For any norm $\norm{\cdot}$ on $\Rd$, there is some constant $\normshellbound{\norm{\cdot}}<\infty$ such that for any $\vect x\in\Rd$ and $0\le a\le b$,% with $b\ge 1$,
\[
\card[1]{\setbuilder[1]{\vect v\in\Zd}{a\le \norm{\vect v-\vect x}\le b}}
\le \normshellbound{\norm{\cdot}} (b\join 1)^{d-1} \brackets[2]{(b-a)\join 1}.
\]
\end{lem}

\begin{proof}
This should be a simple geometric fact\ldots

\underline{Idea:} Let $V$ be the set of lattice points in the statement. Then $\card{V} = \lebmeasof[2]{d}{\cubify{V}}$, so we need to estimate the volume of $\cubify{V}$. What might be helpful is Theorem~2.49 on p.\ 78 of Folland, saying that $d$-dimensional Lebesgue measure can be decomposed into the product of 1-dimensional Lebesgue measure with the surface measure of $\sphere{d-1}{\ltwo{d}}$, and giving a formula for integrals. Maybe we can use some modification of this theorem since $\cubify{V}$ is close to a scaled and thickened version of $\sphere{d-1}{\norm{\cdot}}$.

\end{proof}



\begin{lem}[A bound for ``polynomial$\times$geometric" series]
\label{poly_geo_series_lem}
For any $n\in\N$, $c>0$, and $a,m\ge 0$,
\[
\sum_{j=n}^\infty (j+a)^m e^{-cj}
\le \frac{4}{(c\meet 1)^{m+1}}\cdot  \parens{2m \join a}^m \cdot e^{-\frac{c}{2} n},
\]
with the convention $0^0=1$ when $m=0$.
\end{lem}

\begin{proof}
\newcommand{\xmax}{x_{\max}}
%\newcommand{\fmax}{}

%For $a,m\ge 0$ and $b>0$, the function $f(x) = (x+a)^m e^{-bx}$ attains a global maximum on $[-a,\infty)$ at $\xmax = \frac{m}{b} -a$, and $f(\xmax) = \parens[2]{\frac{m}{ce}}^m e^{ba}$.

%SOURCE: Notes from June 13, 14, 21, 2011
%SEE ALSO: Notes from December 31, 2011; Propositions 2.21, 2.22 in 'fpp_cones.tex'
%ORIGINAL WRITEUP: Jan 15-16, 2012

For any $a,m\ge 0$ and $b>0$, consider the function $f : [-a,\infty)\to \Rplus$ defined by $f(x) = (x+a)^m e^{-bx}$, with the convention $0^0=1$ when $m=0$. Computing $f'(x)$ shows that $f$ attains a global maximum of $f(\xmax) = \parens[2]{\frac{m}{be}}^m e^{ba}$ at $\xmax = \frac{m}{b} -a$, and $f$ is decreasing on $[\xmax,\infty)$. Therefore, if $\xmax\le 0$, then $\restrict{f}{[0,\infty)}$ attains a maximum of $f(0) = a^m$ at $x=0$, so we have
\begin{equation}
\label{poly_geo_series:sup_cases_eqn}
\sup_{x\ge 0}\; (x+a)^m e^{-bx}=
\begin{cases}
\parens[1]{\frac{m}{be}}^m e^{ba} &\text{if } ab\le m,\\
a^m &\text{if } ab\ge m.
\end{cases}
\end{equation}
Note that if $ab\le m$, then $\parens[2]{\frac{m}{be}}^m e^{ba} \le \parens[2]{\frac{m}{be}}^m e^{m} = \parens[1]{\frac{m}{b}}^m$, so \eqref{poly_geo_series:sup_cases_eqn} implies that
\begin{equation}
\label{poly_geo_series:sup_bound_eqn}
\sup_{x\ge 0}\; (x+a)^m e^{-bx} \le
\parens[1]{\frac{m}{b} \join a}^m.
\end{equation}
Using the bound \eqref{poly_geo_series:sup_bound_eqn} with $b=c/2$ and $x=j$, for any $n\in\N$ we get
\begin{align*}
\sum_{j=n}^\infty (j+a)^m e^{-cj}
&= \sum_{j=n}^\infty (j+a)^m e^{-\frac{c}{2}j} e^{-\frac{c}{2}j}\\
&\le \parens[1]{\frac{2m}{c} \join a}^m \cdot \sum_{j=n}^\infty  e^{-\frac{c}{2}j}\\
&= \parens[1]{\frac{2m}{c} \join a}^m \cdot \frac{e^{-\frac{c}{2}n}}{1-e^{-\frac{c}{2}}}\\
&\le \parens[1]{\frac{2m}{c\meet 1} \join a}^m
	\cdot \frac{4}{c\meet 1}\cdot e^{-\frac{c}{2}n}\\
&\le \frac{4}{(c\meet 1)^{m+1}}\cdot \parens{2m \join a}^m
	\cdot e^{-\frac{c}{2}n},
\end{align*}
where in the second-to-last line we have used the bound
\[
\frac{1}{1-e^{-\frac{c}{2}}} = \frac{e^{\frac{c}{2}}}{e^{\frac{c}{2}} - 1}
\le \frac{2}{\parens[2]{e^{\frac{c}{2}} - 1}\meet 1} \le \frac{2}{\parens[1]{\frac{c}{2}}\meet 1}
\le \frac{4}{c\meet 1}. \qedhere
\]
\end{proof}

%%Commented out 2012/1/28:
%%(2012/1/28): Instead of doing this proof directly, I proved it as a short corollary of the "paths in a spherical shell lemma," and put the proof in the main text of Chapter 4.
%\begin{lem}[Lemma~\ref{path_tail_bound_lem}: Traversal of radial lattice paths in a $\mu$-ball]
%%\label{path_tail_bound_lem}
%\newcommand{\thisevent}{\symbolref{\eventsymb}{path_tail_bound_lem}(r)}
%Let $\konstref{path_tail_bound_lem} = \parens[2]{2+\dilnorm{\lspace{\infty}{d}}{\mu}}\konst{\mu}$, where $\konst{\mu}$ is the constant from Lemma~\ref{segment_meas_lem}, and for each $r\ge 0$, define the event
%\[
%\thisevent = \bigcap_{\vect z\in \cubify{\vect 0}} \bigcap_{t\ge r}
%	\eventthat[3]{\tmeasure \parens[2]{\segment{\vect z}{\vect z+ \vect x}}
%	\le \konstref{path_tail_bound_lem} t
%	\text{ for all } \vect x\in \reacheddset{\mu}{\vect 0}{t} }.
%\]
%Then there exist (universal) positive constants $\bigcref{path_tail_bound_lem}$ and $\smallcref{path_tail_bound_lem}$ such that for all $r\ge 0$,
%\[
%\Pr \parens[2]{\thisevent} \ge 
%1-\bigcref{path_tail_bound_lem}e^{-\smallcref{path_tail_bound_lem} r}.
%\]
%\end{lem}
%
%
%\begin{proof}
%\newcommand{\thisevent}{\symbolref{\eventsymb}{path_tail_bound_lem}(r)}
%\newcommand{\thiskonst}{\konstref{path_tail_bound_lem}}
%\newcommand{\thisC}{\bigcref{path_tail_bound_lem}}
%\newcommand{\thisc}{\smallcref{path_tail_bound_lem}}
%
%\newcommand{\thisdil}{\kappa}
%
%For $j\in\N$, define the event
%\begin{align}\label{path_tail_bound:Ej_eqn}
%E_j
%&\definedas \bigcap_{j\le t< j+1} \bigcap_{\vect z\in \cubify{\vect 0}}
%	\eventthat[3]{\tmeasure \parens[2]{\segment{\vect z}{\vect z+ \vect x}}
%	\le \thiskonst t
%	\text{ for all } \vect x\in \reacheddset{\mu}{\vect 0}{t} } \notag\\
%&\supseteq  \bigcap_{j\le t< j+1}
%	\eventthat[3]{\tmeasure \parens[2]{\segment{\vect z}{\vect y}}
%	\le \thiskonst t
%	\text{ for all } \vect z\in\cubify{\vect 0} \text{ and }
%	\vect y\in \cubify{\vect 0} + \reacheddset{\mu}{\vect 0}{t} },
%\end{align}
%and note that $\thisevent \supseteq \bigcap_{j=\floor{r}}^\infty E_j$.
%%Now observe that
%%\[
%%\bigcup_{\vect z\in\cubify{\vect 0}} \bigcup_{\vect x\in  \reacheddset{\mu}{\vect 0}{t}}
%%\setof{\vect z+\vect x} = \cubify{\vect 0} + \reacheddset{\mu}{\vect 0}{t},
%%\]
%%\[
%%\setbuilder[3]{\vect z+\vect x}{\vect z\in \cubify{\vect 0}, \vect x\in \reacheddset{\mu}{\vect 0}{t}}
%%= \cubify{\vect 0} + \reacheddset{\mu}{\vect 0}{t},
%%\]
%%and since $A\subseteq \cubify[2]{\lat A} = \cubify{\vect 0} + \Zd \cap (\cubify{\vect 0} + A)$ for any $A\subseteq\Rd$,
%%\[
%%\vect y\in  \cubify{\vect 0} + \reacheddset{\mu}{\vect 0}{t}
%%\implies
%%\vect y\in \cubify{\vect v} \text{ for some }
%%\vect v\in \Zd \cap \parens[1]{2\cubify{\vect 0} + \reacheddset{\mu}{\vect 0}{t}}
%%\]
%Recall [[cite some lemma]] that  for any $A\subseteq\Rd$,
%\[
%A\subseteq \cubify[2]{\lat A} =
%\bigcup \setbuilder[1]{\cubify{\vect v}}{\vect v \in \Zd \cap (\cubify{\vect 0}+A)}.
%\]
%Taking $A= \cubify{\vect 0} + \reacheddset{\mu}{\vect 0}{t}$, and noting that $\cubify{\vect 0} + \cubify{\vect 0} = \unitball{\lspace{\infty}{d}}$, we get
%\begin{equation}\label{path_tail_bound:lattice_points_eqn}
%\vect y\in  \cubify{\vect 0} + \reacheddset{\mu}{\vect 0}{t}
%\implies
%\vect y\in \cubify{\vect v} \text{ for some }
%\vect v\in \Zd \cap \parens[1]{\unitball{\lspace{\infty}{d}} + \reacheddset{\mu}{\vect 0}{t}}.
%\end{equation}
%%Therefore, noting that $\unitball{\lspace{\infty}{d}} + \reacheddset{\mu}{\vect 0}{t} \subseteq \reacheddset{\mu}{\vect 0}{t+\thisdil}$, where $\thisdil \definedas \dilnorm{\lspace{\infty}{d}}{\mu}$,
%Now note that by the triangle inequality,
%\begin{equation}\label{path_tail_bound:dilatation_eqn}
%\unitball{\lspace{\infty}{d}} + \reacheddset{\mu}{\vect 0}{t}
%\subseteq \reacheddset{\mu}{\vect 0}{t+\thisdil},
%\text{ where } \thisdil \definedas \dilnorm{\lspace{\infty}{d}}{\mu}.
%\end{equation}
%Starting with \eqref{path_tail_bound:Ej_eqn}, and then using \eqref{path_tail_bound:lattice_points_eqn} and \eqref{path_tail_bound:dilatation_eqn} in the second line,
%\begin{align}\label{path_tail_bound:complement_containment}
%E_j^\complement
%&\subseteq \bigcup_{j\le t\le j+1}
%	\eventthat[1]{\tmeasure \parens[2]{\segment{\vect z}{\vect y}} > \thiskonst t
%	\text{ for some $\vect z\in \cubify{\vect 0}$ and 
%	$\vect y\in \cubify{\vect 0}+ \reacheddset{\mu}{\vect 0}{t}$}} \notag\\
%&\subseteq  \bigcup_{j\le t\le j+1} \bigcup_{\substack{\vect v\in \Zd \\ \mu(\vect v)\le t+\thisdil}}
%	\eventthat[1]{\tmeasure \parens[2]{\segment{\vect z}{\vect y}} > \thiskonst t
%	\text{ for some } \vect z\in \cubify{\vect 0} \text{ and }
%	\vect y\in \cubify{\vect v}} \notag\\
%&\subseteq \bigcup_{\substack{\vect v\in \Zd \\ \mu(\vect v)\le j+1+\thisdil}}
%	\eventthat[1]{\tmeasure \parens[2]{\segment{\vect z}{\vect y}} > \thiskonst j
%	\text{ for some } \vect z\in \cubify{\vect 0} \text{ and }
%	\vect y\in \cubify{\vect v}}\\
%&= \bigcup_{\substack{\vect v\in \Zd \\ \mu(\vect v)\le j+1+\thisdil}}
%	\eventref{segment_meas_lem} (\vect 0,\vect v, \thiskonst j)^\complement
%\end{align}
%Now note that
%\[
%j\ge 1 \implies
%\thiskonst j = (2+\thisdil)\konst{\mu}j \ge \konst{\mu} (j+1+\thisdil),
%\]
%and that $\dist{\mu}\parens[2]{\cubify{\vect 0},\cubify{\vect v}}\le j+1+\thisdil$ for any $\vect v\in\Zd$ with $\mu(\vect v)\le j+1+\thisdil$. Therefore, combining \eqref{path_tail_bound:complement_containment} with Lemma~\ref{segment_meas_lem},
%\begin{align}\label{path_tail_bound:complement_bound}
%\forall j\ge 1,\quad& \notag\\
%\Pr \parens[3]{E_j^\complement}
%&\le \sum_{\substack{\vect v\in \Zd \\ \mu(\vect v)\le j+1+\thisdil}}
%	\Pr \eventthat[1]{\tmeasure \parens[2]{\segment{\vect z}{\vect y}} > \konst{\mu} (j+1+\thisdil)
%	\text{ for some } \vect z\in \cubify{\vect 0} \text{ and }
%	\vect y\in \cubify{\vect v}} \notag\\
%&\le \sum_{\substack{\vect v\in \Zd \\ \mu(\vect v)\le j+1+\thisdil}}
%	\bigcref{segment_meas_lem} e^{-\smallcref{segment_meas_lem} (j+1+\thisdil)} \notag\\
%&\le \mushellbound \cdot (j+1+\thisdil)^d\cdot
%	\bigcref{segment_meas_lem} e^{-\smallcref{segment_meas_lem} (j+1+\thisdil)}.
%\end{align}
%Finally, 
%%since $\thisevent^\complement \subseteq \bigcup_{j=\floor{r}}^\infty E_j^\complement$,
%\eqref{path_tail_bound:complement_bound} implies that for any $r\ge 1$,
%\[
%\Pr \parens[3]{\thisevent^\complement}
%\le \sum_{j=\floor{r}}^\infty \Pr \parens[3]{E_j^\complement}
%\le  \sum_{j=\floor{r}}^\infty \mushellbound \cdot (j+1+\thisdil)^d\cdot
%	\bigcref{segment_meas_lem} e^{-\smallcref{segment_meas_lem} (j+1+\thisdil)}
%\le \thisC e^{-\thisc r},
%\]
%where $\thisC$ and $\thisc$ are some positive constants depending only on $\E \mttime_0$ (through the constants $\bigcref{segment_meas_lem}$ and $\smallcref{segment_meas_lem}$), $\mu$, and $d$. By increasing $\thisC$ if necessary, the same bound will trivially work for $0\le r<1$.
%\end{proof}

\begin{lem}[Lemma~\ref{growth_containment_lem}: Containment of growth within large $\mu_2$-balls far from the origin]
%\label{growth_containment_lem}
\newcommand{\thisevent}{\eventref{growth_containment_lem}\parens{r,\beta;\alpha}}
\newcommand{\thiskonst}{k_{\mu_1}}

For any constants $\alpha\in (0,1)$, $\beta\ge 1$, and $r>0$, define the event
\[
\thisevent =
 \bigcap_{\vect z\in \cubify{\vect 0}} \bigcap_{\substack{\vect x\in \Rd \\ \mu_1(\vect x) \ge r}}
\eventthat[1]{ \rreachedset{\tmeasure_2}{\vect z+\vect x}{\Rd}{\alpha t} \subseteq
\reacheddset{\mu_2}{\vect z+\vect x}{t-} \;\forall t\ge \beta \mu_1(\vect x) },
\]
and let $\thiskonst = 3\dilnorm{\lspace{\infty}{d}}{\mu_1}+1$. Then given $\alpha \in (0,1)$, there exist positive constants $C_{\ref{growth_containment_lem}}$ and $c_{\ref{growth_containment_lem}}$ such that for any $\beta\ge 1$ and $r \ge 0$,
\[
\Pr \parens[2]{\thisevent} \ge 1- \bigcref{growth_containment_lem}(\alpha)
e^{-\smallcref{growth_containment_lem}(\alpha)\cdot \beta \cdot (r - \thiskonst)}.
\]
\end{lem}

\begin{proof}
\newcommand{\thisevent}{\eventref{growth_containment_lem}\parens{r,\beta;\alpha}}
\newcommand{\thisC}{\bigcref{growth_containment_lem}(\alpha)}
\newcommand{\thisc}{\smallcref{growth_containment_lem}(\alpha)}

\newcommand{\thiskonst}{k_{\mu_1}}

\newcommand{\ballevent}[4][0]{\eventsymb^{#2} \parens[#1]{#3;#4}}%{\eventsymb^{\vect v}\parens{r;\alpha}}
%{\eventref{strong_dev_cor}}
\newcommand{\Calpha}{\bigcsymb(\alpha)}
\newcommand{\calpha}{\smallcsymb(\alpha)}

\newcommand{\thisz}{\vect z}
\newcommand{\thisy}{\vect y}
\newcommand{\thisx}{\vect x}
\newcommand{\thisv}{\vect v}

\newcommand{\thiscube}{\cubify{\vect 0}}

\newcommand{\thisdil}{\kappa}
\newcommand{\thisshellbound}{\normshellbound{\mu_1}}

%ORIGINAL WRITEUP: Sometime in May, 2011; Jan 20, 2012

Fix $\alpha\in (0,1)$, and for each $\vect v\in\Zd$ and $r\ge 0$, define the event
\[
\ballevent{\thisv}{r}{\alpha} \definedas \bigcap_{\vect y\in \cubify{\vect v}}
\eventthat[1]{\rreachedset{\tmeasure_2}{\thisv}{\Rd}{\alpha t} \subseteq \reacheddset{\mu_2}{\vect y}{t-}
\;\forall t\ge r}.
\]
%[[2012/2/15: Oops, I need to replace $\reachedset{2}{\vect v}{\alpha t}$ with $\rreachedset{\tmeasure_2}{\vect v}{\Rd}{\alpha t}$, and similarly for all other instances of the random process in this lemma.]] Did this on 2012/2/16.
Then $\ballevent{\thisv}{r}{\alpha}\supseteq \eventref{shifted_dev_bounds_lem}^{\thisv} \parens[2]{\alpha r; \alpha^{-1}-1}$, with $\tmeasure = \tmeasure_2$ and $\mu=\mu_2$. Thus, since $\alpha<1$, Lemma~\ref{shifted_dev_bounds_lem} implies there are positive constants $\Calpha$ and $\calpha$ (depending on $\law \parens[2]{\tmeasure_2 (\edge)}$) such that for any $\vect v\in\Zd$ and $r\ge 0$,
\begin{equation}
\label{growth_containment:ballevent_prob_eqn}
\Pr \parens[2]{\ballevent{\thisv}{r}{\alpha}} \ge 1- \Calpha e^{-\calpha r}.
\end{equation}
Let $\thisdil = \dilnorm{\lspace{\infty}{d}}{\mu_1}$. Then using \eqref{space_covering:yz_bounds} and \eqref{space_covering:yv_bounds} (from the proof of Lemma~\ref{space_covering_lem}, with $\mu_1$ in place of $\mu$) in lines three and four, respectively, we have
\begin{align*}
\eventcomplement{\thisevent}
&= \bigcup_{\thisz\in\thiscube} \bigcup_{\substack{\thisx\in\Rd \\ \mu_1(\thisx)\ge r}}
	\eventthat[3]{ \rreachedset{\tmeasure_2}{\thisz+\thisx}{\Rd}{\alpha t} \not\subseteq
	\reacheddset{\mu_2}{\thisz+\thisx}{t-} \text{ for some } t\ge \beta \mu_1(\thisx) }\\
&= \bigcup_{\thisz\in\thiscube} \bigcup_{\substack{\thisy\in\Rd \\ \mu_1(\thisy-\thisz)\ge r}}
	\eventthat[3]{ \rreachedset{\tmeasure_2}{\thisy}{\Rd}{\alpha t} \not\subseteq
	\reacheddset{\mu_2}{\thisy}{t-} \text{ for some } t\ge \beta \mu_1(\thisy-\thisz) }\\
&\subseteq \bigcup_{\substack{\thisy\in\Rd \\ \mu_1(\thisy)\ge r - \thisdil/2}}
	\eventthat[3]{ \rreachedset{\tmeasure_2}{\thisy}{\Rd}{\alpha t} \not\subseteq
	\reacheddset{\mu_2}{\thisy}{t-} \text{ for some }
	t\ge \beta \parens[2]{\mu_1(\thisy) - \thisdil/2} }\\
&\subseteq \bigcup_{\substack{\thisv\in\Zd \\ \mu_1(\thisv)\ge r - \thisdil}}
	\bigcup_{\thisy\in \cubify{\thisv}}
	\eventthat[3]{ \rreachedset{\tmeasure_2}{\thisv}{\Rd}{\alpha t} \not\subseteq
	\reacheddset{\mu_2}{\thisy}{t-} \text{ for some }
	t\ge \beta \parens[2]{\mu_1(\thisv) - \thisdil} }\\
&=\bigcup_{\substack{\thisv\in\Zd \\ \mu_1(\thisv)\ge r - \thisdil}}
	\eventcomplement{\ballevent[2]{\thisv}{\beta \parens[0]{\mu_1(\thisv) - \thisdil}}{\alpha}}.
\end{align*}
Therefore, \eqref{growth_containment:ballevent_prob_eqn} and Lemmas~\ref{norm_shell_lem} and \ref{poly_geo_series_lem} imply that for all $r\ge 0$,
\begin{align*}
\Pr \parens[1]{\eventcomplement{\thisevent}}
&\le \sum_{\substack{\thisv\in\Zd \\ \mu_1(\thisv)\ge r - \thisdil}}
	\Calpha e^{-\calpha \beta \parens{\mu_1(\thisv) - \thisdil}}
	&& \text{(by \eqref{growth_containment:ballevent_prob_eqn})}\\
&\le \sum_{j = \floor{r-\thisdil}\join 0}^\infty
	\sum_{\substack{\thisv\in\Zd \\ j\le \mu_1(\thisv)<j+1}}
	\Calpha e^{-\calpha \beta \parens{\mu_1(\thisv) - \thisdil}}\\
&\le \sum_{j = \floor{r-\thisdil}\join 0}^\infty
	\thisshellbound (j+1)^{d-1}
	\Calpha e^{-\calpha \beta (j - \thisdil)}
	&& \text{(Lem.~\ref{norm_shell_lem})}\\
&\le \thisshellbound \Calpha e^{\calpha \beta \thisdil}
	\cdot \frac{4(2d-2)^{d-1}}{\parens[2]{[\calpha \beta]\meet 1}^d}
	\cdot e^{-\frac{\calpha}{2} \beta \parens{\floor{r-\thisdil}\join 0}}
	&& \text{(Lem.~\ref{poly_geo_series_lem})}\\
&\le \thisshellbound \Calpha e^{\calpha \beta \thisdil}
	\cdot \frac{4(2d-2)^{d-1}}{\parens[2]{\calpha \meet 1}^d}
	\cdot e^{-\frac{\calpha}{2} \beta \parens{r-\thisdil-1}}
	&& \text{($\because \beta\ge 1$)}\\
&= \frac{4\thisshellbound \Calpha(2d-2)^{d-1}}{\parens[2]{\calpha \meet 1}^d}
	\cdot e^{-\frac{\calpha}{2} \beta \parens{r-3\thisdil-1}}\\
&= \thisC e^{-\thisc \beta (r-\thiskonst)},
\end{align*}
where
\[
\thisC \definedas
\frac{4\thisshellbound \Calpha(2d-2)^{d-1}}{\parens[2]{\calpha \meet 1}^d},
\quad\text{and}\quad
\thisc \definedas \frac{\calpha}{2}.
\qedhere
\]
\end{proof}




